Expanding the reach of quantum optimization with fermionic embeddings

Quadratic programming over orthogonal matrices encompasses a broad class of hard optimization problems that do not have an efficient quantum representation. Such problems are instances of the little noncommutative Grothendieck problem (LNCG), a generalization of binary quadratic programs to continuous, noncommutative variables. In this work, we establish a natural embedding for this class of LNCG problems onto a fermionic Hamiltonian, thereby enabling the study of this classical problem with the tools of quantum information. This embedding is accomplished by a new representation of orthogonal matrices as fermionic quantum states, which we achieve through the well-known double covering of the orthogonal group. Correspondingly, the embedded LNCG Hamiltonian is a two-body fermion model. Determining extremal states of this Hamiltonian provides an outer approximation to the original problem, a quantum analogue to classical semidefinite relaxations. In particular, when optimizing over the \emph{special} orthogonal group our quantum relaxation obeys additional, powerful constraints based on the convex hull of rotation matrices. The classical size of this convex-hull representation is exponential in matrix dimension, whereas our quantum representation requires only a linear number of qubits. Finally, to project the relaxed solution back into the feasible space, we propose rounding procedures which return orthogonal matrices from appropriate measurements of the quantum state. Through numerical experiments we provide evidence that this rounded quantum relaxation can produce high-quality approximations.

==> edge_rouding_alg.tex <==
% Not used currently

\begin{algorithm}\label{alg:rounding}
\caption{Rounding edge marginals}
\KwData{$\ket{\psi} \in \mathcal{H}_d^{\otimes m}$}
\KwResult{$R_1, \ldots, R_m \in G$}

$M \gets 0 \in \R^{mn \times mn}$ \;

\For{$u, v \in [m]$}{
    \uIf{$u = v$}{
        $M_{uv} \gets n I$ \;
    }
    \Else{
        \For{$(i, j) \in [n]^2$}{
        $[M_{uv}]_{ij} \gets \ev{\Gamma_{ij}^{(u,v)}}{\psi}$ \;
        }
    }
}

Cholesky decompose $M = LL^\T$ \;
Generate random $S \in \R^{mn \times n}$ with orthonormal columns \;
$\begin{bmatrix}\hat{Q}_1 & \cdots & \hat{Q}_m\end{bmatrix}^\T \gets LS$ \;
\For{$v \in [m]$}{
    $R_v \gets \argmin_{X \in G} \| X - \hat{Q}_v \|_F^2$ \;
}
\end{algorithm}

==> prelims.tex <==


\subsection{\label{sec:clifford_prelim}Clifford algebras and the orthogonal group}

In this section we review the key components for constructing the orthogonal and special orthogonal groups from a Clifford algebra. Our presentation of this material broadly follows Refs.~\cite{atiyah1964clifford,saunderson2015semidefinite}.

% Next we study the Pin and Spin groups and make a number of connections to concepts in quantum information. Most prominently, the Clifford algebra $\Cl(n)$ is a $2^n$-dimensional real vector space equipped with an inner product, and so can be represented by a Hilbert space $\mathcal{H}_{2^n}$ of $n$ qubits. Because multiplication on an algebra is bilinear, it is represented in the Hilbert space by linear operators. The quadratic map $Q$ then corresponds to the expectation values of a collection of these operators (actually, $n$-qubit Pauli operators). We also show that, under this correspondence, the Pin group corresponds to a class of pure free-fermion states (identifying qubits with fermionic modes under the Jordan--Wigner isomorphism). Meanwhile, the Spin group comprises such states with an even number of fermions (even parity).

% Finally, we construct a Hamiltonian whose energy serves as a relaxation to the LNCG objective. The Hamiltonian terms are constructed from the Pauli operators which define the quadratic map $Q$ in this quantum formalism, thus guaranteeing that their expectation values return an orthogonal matrix when the state is a free-fermion state. Otherwise the quadratic map returns an element outside of the orthogonal group (but within the convex hull of the group), which indicates the relaxed property of the Hamiltonian.

The Clifford algebra $\Cl(n)$ of $\R^n$ is a $2^n$-dimensional real vector space, equipped with an inner product $\langle \cdot, \cdot \rangle : \Cl(n) \times \Cl(n) \to \R$ and a multiplication operation satisfying the anticommutation relation
\begin{equation}\label{eq:anticommutator_cl_n}
    e_i e_j + e_j e_i = -2 \delta_{ij} \openone,
\end{equation}
where $\{e_1, \ldots, e_n\}$ is an orthonormal basis of $\R^n$ and $\openone$ is the multiplicative identity of the algebra. The basis elements $e_i$ are called the generators of the Clifford algebra, in the sense that they generate all other basis vectors of $\Cl(n)$ as
\begin{equation}
    e_I \coloneqq e_{i_1} \cdots e_{i_k}, \quad I = \{i_1, \ldots, i_k\} \subseteq [n].
\end{equation}
By convention we order the indices $i_1 < \cdots < i_k$, and the empty set corresponds to the identity, $e_\varnothing = \openone$. Taking all subsets $I \subseteq [n]$ and extending the inner product definition from $\R^n$ to $\Cl(n)$, it follows that $\{e_I \mid I \subseteq [n]\}$ is an orthonormal basis with $2^n$ elements. Specifically, we can write any element $x \in \Cl(n)$ as
\begin{equation}\label{eq:inner_product_cl_n}
    x = \sum_{I \subseteq [n]} x_I e_I
\end{equation}
with each $x_I \in \R$, and the inner product on $\Cl(n)$ is\footnote{\az{Move this to appendix} Equipping an inner product to the vector representation of $\Cl(n)$ elements is achieved using the fact that algebra elements square to a constant.  Each algebra element is orthogonal using the definition of the inner product given in Eq.~\eqref{eq:inner_product_cl_n}.}
\begin{equation}
    \langle x, y \rangle = \sum_{I \subseteq [n]} x_I y_I,
\end{equation}
where $y = \sum_{I \subseteq [n]} y_I e_I$. Hence $\Cl(n)$ is isomorphic as a Hilbert space to $\R^{2^n}$.

Now we show how to realize the orthogonal group $\Orth(n)$ from this algebra. First observe the inclusion $\R^n = \spn\{e_i \mid i \in [n]\} \subset \Cl(n)$. We shall identify the sphere $S^{n-1} \subset \R^n$ as all $u \in \R^n$ satisfying $\langle u, u \rangle = 1$. We then define the Pin group as all possible products of $S^{n-1}$ elements:
\begin{equation}\label{eq:pin}
    \Pin(n) \coloneqq \{u_1 \cdots u_{k} \mid u_1, \ldots, u_{k} \in S^{n-1}, 0 \leq k \leq n\}.
\end{equation}
It is straightforward to check that this is indeed a group. Each $x \in \Pin(n)$ is also normalized, $\langle x, x \rangle = 1$. In fact, an equivalent definition of this group is all elements $x \in \Cl(n)$ satisfying $x \overline{x} = \openone$, where conjugation $\overline{x}$ is defined from the linear extension of
\begin{equation}
    \overline{e_I} \coloneqq (-1)^{|I|} e_{i_k} \cdots e_{i_1}.
\end{equation}
The Pin group is a double cover of $\Orth(n)$, which can be seen from defining a quadratic map $Q : \Cl(n) \to \R^{n \times n}$. This map arises from the so-called twisted adjoint action, introduced by Atiyah \emph{et al.}~\cite{atiyah1964clifford}:
\begin{equation}
    v \mapsto \alpha(x) v \overline{x}, \quad x, v \in \Cl(n),
\end{equation}
where the linear map $\alpha : \Cl(n) \to \Cl(n)$ is the parity automorphism, defined by linearly extending
\begin{equation}
    \alpha(e_I) \coloneqq (-1)^{|I|} e_I.
\end{equation}
Then for any $x \in \Cl(n)$, the linear map $Q(x) : \R^n \to \R^n$ is defined as
\begin{equation}\label{eq:quad_map_clifford}
    Q(x)(v) \coloneqq \pi_{\R^n}(\alpha(x) v \overline{x}) \quad \forall v \in \R^n,
\end{equation}
where $\pi_{\R^n}$ is the projection from $\Cl(n)$ onto $\R^n$. To show that $Q(\Pin(n)) = \Orth(n)$, it suffices to recognize that, for any $u \in S^{n-1}$, $\alpha(u) v \overline{u} \in \R^n$ is the reflection of the vector $v \in \R^n$ across the hyperplane normal to $u$. Then by the Cartan--Dieudonn{\'e} theorem one can implement any orthogonal transformation on $\R^n$ by composing $k \leq n$ such reflections about arbitrary hyperplanes $u_1, \ldots, u_k$~\cite{gallier2011geometric}. This characterization coincides precisely with the definition of the Pin group provided in Eq.~\eqref{eq:pin}. Hence for all $x \in \Pin(n)$, $Q(x)$ is an orthogonal transformation on $\R^n$. The double cover property follows from the fact that $Q$ is quadratic in $x$, so $Q(x) = Q(-x)$. 

The special orthogonal group arises from the subgroup $\Spin(n) \subset \Pin(n)$ containing only even-parity Clifford elements. First observe that $\Cl(n)$ is a $\Z_2$-graded algebra:
\begin{equation}
    \Cl(n) = \Cl^{0}(n) \oplus \Cl^{1}(n),
\end{equation}
where
\begin{align}
    \Cl^0(n) &\coloneqq \spn\{e_I \mid |I| \text{ even}\},\\
    \Cl^1(n) &\coloneqq \spn\{e_I \mid |I| \text{ odd}\}.
\end{align}
By a $\Z_2$ grading we mean that for each $x \in \Cl^a(n)$ and $y \in \Cl^b(n)$, their product $xy$ lies in $\Cl^{a + b \mod 2}(n)$. We say that elements in $\Cl^0(n)$ (resp., $\Cl^1(n)$) have even (resp., odd) parity. In particular, this grading implies that $\Cl^{0}(n)$ is a subalgebra, hence its intersection with the Pin group is also a group, which defines
\begin{equation}
    \Spin(n) \coloneqq \Pin(n) \cap \Cl^{0}(n) = \{u_1 \cdots u_{2k} \mid u_1, \ldots, u_{2k} \in S^{n-1}, 0 \leq k \leq \lfloor n/2 \rfloor\}.
\end{equation}
Just as the Pin group double covers $\Orth(n)$, so does the Spin group double cover $\SO(n)$. This is again a consequence of the Cartan--Dieudonn{\'e} theorem, wherein all rotations on $\R^n$ can be decomposed into an even number of (at most $n$) arbitrary reflections.

\subsection{The convex hull of the (special) orthogonal group}

The convex hull $\conv S$ of a set $S$ is the set of all convex combinations of elements of $S$. If $S$ is a nonconvex space, optimization over its elements may be difficult, even when the objective itself is a convex function. However, the relaxed problem over $\conv S$ enjoys many nice properties of convex optimization.
%In particular, suppose the convex set $C \subset \R^N$ can be expressed in the form
% \begin{equation}\label{eq:spectrahedron}
%     C = \l\{ x \in \R^N \mathrel{\Bigg|} \I_m + \sum_{i \in [N]} x_i A_i \succeq 0 \r\}
% \end{equation}
% for some real symmetric $m \times m$ matrices $A_1, \ldots, A_N$. Then $C$ is called a spectrahedron, which is the intersection of the cone of positive semidefinite (PSD) matrices with a linear affine subspace. Spectrahedra constitute the feasible regions of semidefinite programs (SDPs), which are convex optimization problems that can be solved in polynomial time to arbitrary precision. The description of Eq.~\eqref{eq:spectrahedron} is called a spectrahedral representation of $C$ of size $m$.
This observation motivates the study of the convex hull of orthogonal matrices, $\conv\Orth(n)$ and $\conv\SO(n)$. The latter is the focus of Saunderson \emph{et al.}~\cite{saunderson2015semidefinite}, and here we review the main results of that work.

For any $X \in \R^{n \times n}$, let $X = U \Sigma V^\T$ be its singular value decomposition, where $U, V \in \Orth(n)$ and by convention the singular values $\Sigma = \mathrm{diag}(\sigma_1(X), \ldots, \sigma_n(X))$ are in descending order, $\sigma_1(X) \geq \cdots \geq \sigma_n(X) \geq 0$. We also make us of the special singular value decomposition $X = U \widetilde{\Sigma} \widetilde{V}^\T$, where $\widetilde{\Sigma} \coloneqq \Sigma J$ are called the special singular values, $\widetilde{V} \coloneqq VJ$, and $J \in \R^{n \times n}$ is the diagonal matrix
\begin{equation}
    J \coloneqq \begin{bmatrix}
    \I_{n-1} & 0\\
    0 & \det(UV^\T)
    \end{bmatrix}.
\end{equation}
The special singular values potentially differ from the singular values only in the $n$th spot, $\widetilde{\sigma}_n(X) = \det(UV^\T) \sigma_n(X)$. This decomposition is valuable in the context of working with the special orthogonal group, as it guarantees that $U \widetilde{V}^\T \in \SO(n)$.

% This decomposition is motivated by considering the symmetries of $\SO(n)$. Define the group action of $\Orth(n) \times \Orth(n)$ on $\R^{n \times n}$ as $(U, V) \cdot X \coloneqq U X V^\T$. Clearly, $\Orth(n)$ is invariant under this action. On the other hand, $\SO(n)$ is invariant under the action of a subgroup,
% \begin{equation}
%     \mathrm{S}(\Orth(n) \times \Orth(n)) \coloneqq \{ (U, V) \in \Orth(n) \times \Orth(n) \mid \det(U)\det(V) = 1 \}.
% \end{equation}
% Importantly, these symmetries are preserved by the convex hulls of $\Orth(n)$ and $\SO(n)$ as well. Thus the elements of $\conv\Orth(n)$ and $\conv\SO(n)$ can be fully characterized by their (special) singular values alone.

The convex hull of $\Orth(n)$ is the unit operator-norm ball in $\R^{n \times n}$,
\begin{equation}
    \conv\Orth(n) = \l\{ X \in \R^{n \times n} \mid \sigma_1(X) \leq 1 \r\}.
\end{equation}
% This convex body has a well-known spectrahedral representation of size $2n$,
% \begin{equation}\label{eq:convOn}
%     \conv\Orth(n) = \l\{ X \in \R^{n \times n} \mathrel{\Bigg|}
%     \begin{bmatrix}
%     0 & X\\
%     X^\T & 0
%     \end{bmatrix}
%     \preceq \I_{2n} \r\}.
% \end{equation}
% A spectrahedron is the intersection of the cone of positive semidefinite (PSD) matrices with a linear affine subspace, thus defining the feasible region of a semidefinite program. A convex shape has a spectrahedral representation of size $N$ if it can be described as a spectrahedron over $N \times N$ PSD matrices.
On the other hand, the convex hull of $\SO(n)$ has a more complicated description in terms of special singular values:
% A corollary of Horn's theorem~\cite{horn1954doubly} provides a characterization based on the special singular value decomposition:
\begin{equation}\label{eq:convSOn_singval}
    \conv\SO(n) = \l\{ X \in \R^{n \times n} \mathrel{\Bigg|} \sum_{i \in [n] \setminus I} \widetilde{\sigma}_i(X) - \sum_{i \in I} \widetilde{\sigma}_i(X) \leq n - 2 \quad \forall I \subseteq [n], |I| \text{ odd} \r\}.
\end{equation}
% To obtain a semidefinite description, consider $\SO^{-}(n) \coloneqq \{ X \in \Orth(n) \mid \det(X) = -1 \}$. Its polar set is the convex body
% \begin{equation}
%     \SO^{-}(n)^\circ \coloneqq \{ Y \in \R^{n \times n} \mid \langle Y, X \rangle \leq 1 \quad \forall X \in \SO^{-}(n) \},
% \end{equation}
% which can be shown to possess a spectrahedral representation of size $2^{n-1}$ as
% \begin{equation}
%     \SO^{-}(n)^\circ = \l\{ Y \in \R^{n \times n} \mathrel{\Bigg|} \sum_{i,j \in [n]} [\mathcal{R} Y]_{ij} \widetilde{P}_{ij} \preceq \I_{2^{n-1}} \r\}.
% \end{equation}
% Here, $\mathcal{R} \in \SO^{-}(n)$ is any fixed reflection matrix, for instance $\mathcal{R} = \mathrm{diag}(1, \ldots, 1, -1)$. The matrices $\widetilde{P}_{ij} \in \R^{2^{n-1} \times 2^{n-1}}$ are defined by
% \begin{equation}
%     \widetilde{P}_{ij} \coloneqq -\Pi_0 \lambda_i \rho_j \Pi_0^\T,
% \end{equation}
% where the matrices $\lambda_i, \rho_j \in \R^{2^n \times 2^n}$ and $\Pi_0 \in \R^{2^{n-1} \times 2^n}$ can be represented as\footnote{Here we use compact quantum notation where $X, Y, Z$ are the $2 \times 2$ Pauli matrices and $\ket{\pm} \coloneqq (\ket{0} \pm \ket{1}) / \sqrt{2})$. These matrix representations can be obtained from the Clifford algebra approach reviewed in Section~\ref{sec:clifford_prelim};~we provide a more detailed presentation, with connections to concepts in quantum information, in Section~\ref{sec:quantum_formalism}.}
% \begin{align}
%     \lambda_i &= Z^{\otimes (i - 1)} \otimes (-\i Y) \otimes \I_2^{\otimes (n - i)},\\
%     \rho_i &= \I_2^{\otimes (i - 1)} \otimes (-\i Y) \otimes Z^{\otimes (n - i)}\\
%     \Pi_0 &= \frac{1}{\sqrt{2}} \l( \bra{+} \otimes \I_2^{\otimes (n-1)} + \bra{-} \otimes Z^{\otimes (n-1)} \r).
% \end{align}
% Observe that $\SO^{-}(n)^\circ$ is also invariant under the action of $\mathrm{S}(\Orth(n) \times \Orth(n))$. Using this symmetry combined with the description of $\conv\SO(n)$ given in Eq.~\eqref{eq:convSOn_singval} in terms of special singular values, Sauderson \emph{et al.}~\cite{saunderson2015semidefinite} show that
% \begin{equation}\label{eq:SO-polar}
%     \conv\SO(n) = \conv\Orth(n) \cap (n - 2) \SO^{-}(n)^\circ,
% \end{equation}
% which combined with Eqs.~\eqref{eq:convOn} and \eqref{eq:SO-polar} yields a spectrahedral representation of $\conv\SO(n)$ of size $2^{n-1} + 2n$,
% \begin{equation}
%     \conv\SO(n) = \l\{ X \in \R^{n \times n} \mathrel{\Bigg|}
%     \begin{bmatrix}
%     0 & X\\
%     X^\T & 0
%     \end{bmatrix}
%     \preceq \I_{2n}, \quad \sum_{i,j \in [n]} [\mathcal{R} X]_{ij} \widetilde{P}_{ij} \preceq (n - 2) \I_{2^{n-1}} \r\}.
% \end{equation}
% The size of this spectrahedral representation is in fact minimal. However, there is a dual representation of $\conv\SO(n)$ as the projection of the set of $2^{n-1} \times 2^{n-1}$ PSD matrices with unit trace, called a PSD lift:
The main result of Saunderson \emph{et al.}~\cite{saunderson2015semidefinite} establishes that this convex body is a spectrahedron, and it can be described by symmetric matrices of dimension $2^{n-1} + 2n$. In fact, they prove that this size is minimal for any spectrahedral representation of $\conv\SO(n)$. For this paper, however, we will be more interested in a dual representation called the positive-semidefinite (PSD) lift of size $2^{n-1}$:
\begin{equation}\label{eq:conv-son_psd-lift}
    \conv\SO(n) = \l\{
    \begin{bmatrix}
    \langle \widetilde{P}_{11}, \varrho \rangle & \cdots & \langle \widetilde{P}_{1n}, \varrho \rangle\\
    \vdots & \ddots & \vdots\\
    \langle \widetilde{P}_{n1}, \varrho \rangle & \cdots & \langle \widetilde{P}_{nn}, \varrho \rangle
    \end{bmatrix}
    \mathrel{\Bigg|} \varrho \succeq 0, \tr \varrho = 1 \r\}.
\end{equation}
The $2^{n-1} \times 2^{n-1}$ matrices $\widetilde{P}_{ij}$ are defined as
\begin{equation}
    \widetilde{P}_{ij} \coloneqq -\Pi_0 \lambda_i \rho_j \Pi_0^\T,
\end{equation}
where the matrices $\lambda_i, \rho_j \in \R^{2^n \times 2^n}$ and $\Pi_0 \in \R^{2^{n-1} \times 2^n}$ can be represented as\footnote{Here we use compact quantum notation where $X, Y, Z$ are the $2 \times 2$ Pauli matrices and $\ket{\pm} \coloneqq (\ket{0} \pm \ket{1}) / \sqrt{2})$. These matrix representations can be obtained from the Clifford algebra approach reviewed in Section~\ref{sec:clifford_prelim};~we provide a more detailed presentation, with connections to concepts in quantum information, in Section~\ref{sec:quantum_formalism}.}
\begin{align}
    \lambda_i &= Z^{\otimes (i - 1)} \otimes (-\i Y) \otimes \I_2^{\otimes (n - i)},\\
    \rho_i &= \I_2^{\otimes (i - 1)} \otimes (-\i Y) \otimes Z^{\otimes (n - i)},\\
    \Pi_0 &= \frac{1}{\sqrt{2}} \l( \bra{+} \otimes \I_2^{\otimes (n-1)} + \bra{-} \otimes Z^{\otimes (n-1)} \r).
\end{align}
While tight lower bounds on the sizes of PSD lifts are less understood, Saunderson \emph{et al.}~\cite{saunderson2015semidefinite} show that for $n \geq 8$ any PSD lift of $\conv\SO(n)$ which respects a symmetry related to the special singular value decomposition must have size at least $\frac{1}{n + 1} 2^{0.54n}$.

% Using the fact that $\SO(n) = Q(\Spin(n))$, hence $\conv\SO(n) = \conv Q(\Spin(n))$, we can understand this PSD representation as the convexification of vectors in $\Spin(n)$ in the same sense that density matrices (mixed quantum states) are convexifications of rays (pure quantum states) in Hilbert space.

\subsection{\label{sec:sdp}Semidefinite relaxations}

Given a maximization problem of some function $f : S \to \R$, a relaxation consists of a set $S' \supseteq S $ and a function $f' : S' \to \R$ such that $f'(x) \geq f(x)$ for all $x \in S$. A standard approach to approximating Problem~\eqref{eq:LNCG} is a relaxation based on the following equivalence:
\begin{equation}\label{eq:LNCG_SD}
    \argmax_{\mathbf{R} \in \Orth(n)^m} \sum_{(u, v) \in E} \langle C_{uv}, R_u R_v^\T \rangle = \argmax_{M \in \R^{mn \times mn}} \langle C, M \rangle \quad \text{subject to } \begin{cases}
    M \succeq 0,\\
    M_{vv} = \I_n & \forall v \in [m],\\
    \mathrm{rank}(M) = n.
    \end{cases}
\end{equation}
Note that this reformulation adjusts the objective value as
\begin{equation}
    \langle C, M \rangle = 2 \sum_{(u, v) \in E} \langle C_{uv}, R_u R_v^\T \rangle + \tr(C).
\end{equation}
The new constraints guarantee that the solution takes the form $M = \mathbf{R} \mathbf{R}^\T$, where we write $\mathbf{R}$ as an $mn \times n$ matrix
\begin{equation}
    \mathbf{R} = \begin{bmatrix}
    R_1\\
    \vdots\\
    R_m
    \end{bmatrix}, \quad R_v \in \Orth(n).
\end{equation}
The rank constraint, being nonconvex in $M$, is the only difficult constraint in this reformulation. By dropping it we relax the problem to a tractable semidefinite program (SDP), which can be solved in polynomial time to arbitrary precision:
\begin{equation}\label{eq:LCG_relaxed}
    \max_{M \in \R^{mn \times mn}} \langle C, M \rangle \quad \text{subject to } \begin{cases}
    M \succeq 0,\\
    M_{vv} = \I_n & \forall v \in [m].
    \end{cases}
\end{equation}

In order to recover a feasible solution to the original problem from the relaxed solution, one performs a rounding procedure on $M$. Bandeira \emph{et al.}~\cite{bandeira2016approximating} study a randomized rounding protocol which can be understood as an $n$-dimensional generalization of the Goemans--Williamson (GW) algorithm~\cite{goemans1995improved} (recall that the Max-Cut problem is an instance of the $n = 1$ case). First, observe that we can write the relaxed solution as $M = \mathbf{X} \mathbf{X}^\T$, where $\mathbf{X}$ is an $mn \times mn$ matrix of the form
\begin{equation}
    \mathbf{X} = \begin{bmatrix}
    X_1\\
    \vdots\\
    X_m
    \end{bmatrix}, \quad X_v \in \R^{n \times mn}.
\end{equation}
This can be accomplished, for instance, by performing a Cholesky decomposition. An equivalent formulation of the SDP~\eqref{eq:LNCG_SD} is therefore
\begin{equation}\label{eq:LNCG_relax}
    \max_{X_1, \ldots, X_m \in \R^{n \times mn}} \sum_{(u, v) \in E} \langle C_{uv}, X_u X_v^\T \rangle \quad \text{subject to} \quad X_v X_v^\T = \I_n \quad \forall v \in [m].
\end{equation}
To round the matrices $X_1, \ldots, X_m$ into orthogonal matrices, Bandeira \emph{et al.}~\cite{bandeira2016approximating} propose the following randomized algorithm with a constant-factor guarantee on the approximation ratio.
\begin{alg}[{\cite[Algorithm 3]{bandeira2016approximating}}]\label{thm:orth-cut_alg}
    Compute $X_1, \ldots, X_n \in \R^{n \times mn}$ a solution to Problem~\eqref{eq:LNCG_relax}. Let $Z$ be an $mn \times n$ Gaussian random matrix whose entries are drawn i.i.d.~from $\mathcal{N}(0, 1/n)$. Return the orthogonal matrices
    \begin{equation}
        O_v = \mathcal{P}(X_v Z),
    \end{equation}
    where $\mathcal{P}(X) \coloneqq \argmin_{Y \in \Orth(n)} \| Y - X \|_F$.
\end{alg}
Note that the value of $\mathcal{P}(X)$ can be efficiently computed from the singular value decomposition of $X = U \Sigma V^\T$ as
\begin{equation}
    \mathcal{P}(X) = UV^\T.
\end{equation}
For any $C \succeq 0$, the rounded solutions are guaranteed to obey
\begin{equation}
    \E\l[ \sum_{(u, v) \in E} \langle C_{uv}, O_u O_v^\T \rangle \r] \geq \alpha_{\Orth(n)}^2 \max_{R_1, \ldots, R_m \in \Orth(n)} \sum_{(u, v) \in E} \langle C_{uv}, R_u R_v^\T \rangle,
\end{equation}
where the expectation is with respect to the Gaussian random $mn \times n$ matrix $Z$, and the approximation ratio $\alpha_{\Orth(n)}^2$ corresponds to the expected average singular value of the Gaussian random $n \times n$ matrix $Z_1 \sim \mathcal{N}(0, \I_n / n)$,
\begin{equation}
    \alpha_{\Orth(n)} \coloneqq \E\l[ \frac{1}{n} \sum_{i \in [n]} \sigma_i(Z_1) \r].
\end{equation}
The choice of random Gaussian matrix $Z$ is a direct ($n \times n$)-matrix generalization of the random unit vector employed in the GW algorithm. Indeed, one can show that this procedure is equivalent to rounding according to $n$ uniformly drawn orthogonal unit vectors from $\R^{mn}$. When $n = 1$ we have that $\frac{Z}{\|Z\|_2} \in \R^m$ is drawn uniformly from the unit sphere and
\begin{equation}
    \alpha_{\Orth(1)}^2 = \frac{2}{\pi},
\end{equation}
which matches the result of Nesterov~\cite{nesterov1998semidefinite} for approximating the commutative problem~\eqref{eq:LCG}. Furthermore, Bandeira \emph{et al.}~\cite{bandeira2016approximating} show that this approximation ratio matches the integrality gap of the relaxation~\eqref{eq:LNCG_relax}, implying that their rounding algorithm applied to this SDP is tight.

Additional convex constraints may be added to the SDP~\eqref{eq:LCG_relaxed} to improve its performance, especially when restricting the optimization over rotations. Saunderson \emph{et al.}~\cite{saunderson2014semidefinite} propose such an augmented SDP using their semidefinite description of $\conv\SO(n)$. First, they show that the problem
\begin{equation}
    \max_{M \in \R^{mn \times mn}} \langle C, M \rangle \quad \text{subject to } \begin{cases}
    M \succeq 0,\\
    M_{vv} = \I_n & \forall v \in [m],\\
    \mathrm{rank}(M) = n,\\
    M_{uv} \in \conv\SO(n) & \forall u, v \in [m]
    \end{cases}
\end{equation}
guarantees that the solution $M = \mathbf{R} \mathbf{R}^\T$ returns $\mathbf{R} \in \SO(n)^m$. Dropping the rank constraint, they arrive at a $\conv\SO(n)$-based relaxation,
\begin{equation}\label{eq:LNCG_SD_conv}
    \max_{M \in \R^{mn \times mn}} \langle C, M \rangle \quad \text{subject to } \begin{cases}
    M \succeq 0,\\
    M_{vv} = \I_n & \forall v \in [m],\\
    M_{uv} \in \conv\SO(n) & \forall u, v \in [m],
    \end{cases}
\end{equation}
which is also an SDP. However, we point out that such semidefinite descriptions of $\conv\SO(n)$ are exponentially large in $n$.

When the blocks $M_{uv} \notin \SO(n)$, one can round them by computing
\begin{equation}
    R_v = \widetilde{\mathcal{P}}(M_{1v}) = \argmin_{Y \in \SO(n)} \|Y - M_{1v} \|_F,
\end{equation}
where the modified projection to $\SO(n)$ is efficiently computed as
\begin{equation}
    \widetilde{\mathcal{P}}(X) = U \widetilde{V}^\T
\end{equation}
from the special singular value decomposition of $X = U \widetilde{\Sigma} \widetilde{V}^\T$. Note that this rounding procedure is deterministic, and it fixes the global rotation degree of freedom by setting $R_1 = \I_n$. Although the rigorous approximation quality for this enhanced SDP is not known, Saunderson \emph{et al.}~\cite{saunderson2014semidefinite} show that it is exact when the graph is a tree. Furthermore, they provide strong numerical evidence that this $\conv\SO(n)$-based relaxation is significantly more powerful than the SDP of Eq.~\eqref{eq:LCG_relaxed} when optimizing over rotation matrices~\cite{saunderson2014semidefinite}.

\subsection{Free fermions}

Because our quantum formalism of Problem~\eqref{eq:LNCG} is closely connected to aspects of fermionic quantum information, here we review standard concepts about free fermions. A system of $n$ fermionic modes, described by the creation operators $a_1^\dagger, \ldots, a_n^\dagger$, can be equivalently represented by the $2n$ Majorana operators
\begin{align}
    \gamma_i &= a_i + a_i^\dagger,\\
    \widetilde{\gamma}_i &= -\i(a_i - a_i^\dagger),
\end{align}
for all $i \in [n]$. %\footnote{In this paper we denote the imaginary unit by $\i \coloneqq \sqrt{-1}$.}
These operators form a representation for the Clifford algebra $\Cl(2n)$, as can be seen by their anticommutation relations,\footnote{Note that we adopt the physicist's convention for the Majorana operators, which takes the generators to be Hermitian, as opposed to Eq.~\eqref{eq:anticommutator_cl_n} wherein they square to $-\openone$.}
\begin{align}
    \gamma_i \gamma_j + \gamma_j \gamma_i = \widetilde{\gamma}_i \widetilde{\gamma}_j + \widetilde{\gamma}_j \widetilde{\gamma}_i &= 2 \delta_{ij} \openone,\\
    \gamma_i \widetilde{\gamma}_j + \widetilde{\gamma}_j \gamma_i &= 0.
\end{align}
The Jordan--Wigner mapping allows us to identify this fermionic system with an $n$-qubit system via the relations
\begin{align}
    \gamma_{i} &= Z^{\otimes (i - 1)} \otimes X \otimes \I_2^{\otimes (n - i)}, \label{eq:gamma_X}\\
    \widetilde{\gamma}_i &= Z^{\otimes (i - 1)} \otimes Y \otimes \I_2^{\otimes (n - i)}, \label{eq:gamma_Y}
\end{align}
where $X, Y, Z$ are the usual single-qubit Pauli matrices. While other mappings exist, this choice is particularly convenient because the binary representation of fermionic occupation numbers maps directly onto that of $n$-qubit states in their computational basis. We therefore work with the two representations interchangeably.

Operators which are quadratic in the Majorana operators (equivalently, the creation and annihilation operators) are called one-body fermionic operators and correspond to the physics of noninteracting fermions. Namely, free-fermion Hamiltonians take the form
\begin{equation}\label{eq:quadratic_majorana_hamiltonian}
    H = \i \sum_{i,j \in [n]} \l( A_{ij} \widetilde{\gamma}_i \widetilde{\gamma}_j + B_{ij} \gamma_i \gamma_j + C_{ij} \widetilde{\gamma}_i \gamma_j \r).
\end{equation}
Note the presence of the imaginary unit, which is required to ensure Hermiticity since we take the convention that $A, B, C \in \R^{n \times n}$. Such Hamiltonians can be diagonalized efficiently by classical methods.

The central tool which makes free-fermion models solvable is the Bogoliubov transformation. Let $O \in \Orth(2n)$, and arrange the Majorana operators into the $2n$-length column vector
\begin{equation}
    \bm{\gamma} \coloneqq \begin{bmatrix}
    \widetilde{\gamma}_1 & \cdots & \widetilde{\gamma}_n & \gamma_1 & \cdots & \gamma_n
    \end{bmatrix}^\T.
\end{equation}
The transformation $\bm{\gamma} \mapsto O \bm{\gamma}$ preserves the fermionic anticommutation relations, so $O \bm{\gamma}$ is another valid set of Majorana operators. At the level of the Hilbert space, these transformations are achieved by fermionic Gaussian unitaries, which correspond to dynamics generated by free-fermion Hamiltonians,\footnote{Strictly speaking, only $\SO(2n)$ transformations are achievable by free-fermion evolution;~a reflection operator is required to reach $\Orth(2n)$, for instance the action of $\gamma_1$.} and are equivalent to matchgate circuits on qubits under the Jordan--Wigner mapping~\cite{knill2001fermionic,terhal2002classical,jozsa2008matchgates}. We denote fermionic Gaussian unitaries by the representation $\mathcal{U} : \Orth(2n) \to \U(2^n)$, which has the adjoint action
\begin{align}
    \mathcal{U}_O \widetilde{\gamma}_i \mathcal{U}_O^\dagger &= [O \bm{\gamma}]_{i} = \sum_{j \in [n]} \l( [O_{11}]_{ij} \widetilde{\gamma}_j + [O_{12}]_{ij} \gamma_j \r), \label{eq:gamma_tilde_gaussian}\\
    \mathcal{U}_O \gamma_i \mathcal{U}_O^\dagger &= [O \bm{\gamma}]_{i + n} = \sum_{j \in [n]} \l( [O_{21}]_{ij} \widetilde{\gamma}_j + [O_{22}]_{ij} \gamma_j \r). \label{eq:gamma_gaussian}
\end{align}
For convenience we have expressed $O \in \Orth(2n)$ as a block matrix,
\begin{equation}\label{eq:O_block}
    O = \begin{bmatrix}
    O_{11} & O_{12}\\
    O_{21} & O_{22}
    \end{bmatrix}.
\end{equation}
If $\det O = 1$, then $\mathcal{U}_O$ commutes with the parity operator $\prod_{i \in [n]} \i \widetilde{\gamma}_i \gamma_i = Z^{\otimes n}$ and so it preserves the parity of the states it acts on. If instead $\det O = -1$, then $\mathcal{U}_O$ and $Z^{\otimes n}$ anticommute and so the unitary maps flips the parity of states.

The block structure of Eq.~\eqref{eq:O_block} will be especially convenient for our purposes, for instance because orthogonal matrices which are block diagonal do not mix between the $\gamma$- and $\widetilde{\gamma}$-type Majorana operators. Therefore, by a slight abuse of notation, it is useful to define
\begin{equation}
    \mathcal{U}_{(U, V)} \coloneqq \mathcal{U}_W, \quad \text{where } W \coloneqq \begin{bmatrix}
    U & 0\\
    0 & V
    \end{bmatrix},
\end{equation}
which can be viewed as the restricted mapping $\Orth(n) \times \Orth(n) \to \U(2^n)$ under the natural inclusion $\Orth(n) \times \Orth(n) \subset \Orth(2n)$. Finally, we point out that the adjoint action defined in Eqs.~\eqref{eq:gamma_tilde_gaussian} and \eqref{eq:gamma_gaussian} is an antihomomorphism,
\begin{equation}
    \mathcal{U}_{O_2} \mathcal{U}_{O_1} (\cdot) \mathcal{U}_{O_1}^\dagger \mathcal{U}_{O_2}^\dagger = \mathcal{U}_{O_1 O_2} (\cdot) \mathcal{U}_{O_1 O_2}^\dagger
\end{equation}
for all $O_1, O_2 \in \Orth(2n)$, and it preserves group inverses,
\begin{equation}
    \mathcal{U}_O^\dagger (\cdot) \mathcal{U}_O = \mathcal{U}_{O^\T} (\cdot) \mathcal{U}_{O^\T}^\dagger.
\end{equation}

Free-fermion, or fermionic Gaussian, states correspond to the ground and thermal states of noninteracting Hamiltonians. A Hamiltonian-free characterization of these states is in their one-body covariance matrices:~for any $n$-mode density matrix $\rho$, we define its covariance matrix $K(\rho)$ as the real antisymmetric $2n \times 2n$ matrix
\begin{equation}
    K(\rho) \coloneqq \begin{bmatrix}
    K_{11}(\rho) & K_{12}(\rho)\\
    K_{21}(\rho) & K_{22}(\rho)
    \end{bmatrix},
\end{equation}
where each block is
\begin{align}
    [K_{11}(\rho)]_{ij} &\coloneqq \frac{1}{2} \tr(\i [\widetilde{\gamma}_i, \widetilde{\gamma}_j] \rho)\\
    [K_{22}(\rho)]_{ij} &\coloneqq \frac{1}{2} \tr(\i [\gamma_i, \gamma_j] \rho)\\
    [K_{12}(\rho)]_{ij} &\coloneqq \frac{1}{2} \tr(\i \widetilde{\gamma}_i \gamma_j \rho) = -[K_{21}(\rho)]_{ji}.
\end{align}
The state $\rho$ is Gaussian if and only if all its higher-body moments are determined by the one-body information in $K(\rho)$ via Wick's theorem. For every valid density matrix we have that $K(\rho)^\T K(\rho) \preceq \I_{2n}$, with equality holding when the Gaussian state $\rho$ is pure. The action of fermionic Gaussian unitaries on states is also conveniently represented using their covariance matrices, as the two states $\rho$ and $\mathcal{U}_O \rho \mathcal{U}_O^\dagger$ have covariance matrices are related by
\begin{equation}
    K(\mathcal{U}_O \rho \mathcal{U}_O^\dagger) = O^\T K(\rho) O.
\end{equation}
